NAS-Bench-360: Benchmarking Neural Architecture Search on Diverse Tasks

Most existing neural architecture search (NAS) benchmarks and algorithms prioritize well-studied tasks, e.g. image classification on CIFAR or ImageNet. This makes the performance of NAS approaches in more diverse areas poorly understood. In this paper, we present NAS-Bench-360, a benchmark suite to evaluate methods on domains beyond those traditionally studied in architecture search, and use it to address the following question: do state-of-the-art NAS methods perform well on diverse tasks? To construct the benchmark, we curate ten tasks spanning a diverse array of application domains, dataset sizes, problem dimensionalities, and learning objectives. Each task is carefully chosen to interoperate with modern CNN-based search methods while possibly being far-afield from its original development domain. To speed up and reduce the cost of NAS research, for two of the tasks we release the precomputed performance of 15,625 architectures comprising a standard CNN search space. Experimentally, we show the need for more robust NAS evaluation of the kind NAS-Bench-360 enables by showing that several modern NAS procedures perform inconsistently across the ten tasks, with many catastrophically poor results. We also demonstrate how NAS-Bench-360 and its associated precomputed results will enable future scientific discoveries by testing whether several recent hypotheses promoted in the NAS literature hold on diverse tasks. NAS-Bench-360 is hosted at https://nb360.ml.cmu.edu.

==> intro_tmp.tex <==
% !TEX root = main.tex

\section{Introduction}\label{sec:intro}

Neural architecture search (NAS) aims to automate the design of deep neural networks, ensuring performance on par with hand-crafted architectures while reducing human labor devoted to tedious architecture tuning \citep{elsken2019nas}. 
With the growing number of application areas of ML, and thus of use-cases for automating it, NAS has experienced an intense amount of study in well-established machine learning domains, with significant progress in search space design~\citep{zoph2018nas,liu2019darts,cai2019proxyless}, search efficiency~\citep{pham2018enas}, and search algorithms~\citep{xu2020pcdarts,li2021gaea,white2021bananas}.
Notably, the field has largely been dominated by methods designed for and evaluated on benchmarks in computer vision \citep{liu2019darts,ying2019nasbench101,dong2020nasbench201}, yet the use of NAS techniques may be especially impactful in under-explored or under-resourced domains where less is known about useful architecture design patterns. 
There have been a few recent efforts to diversify these benchmarks to settings such as vision-based transfer learning \citep{duan2021transnas} and speech and language processing \cite{mehrotra2021asr,klyuchnikov2020nlp};
however, evaluating NAS methods on such well-studied tasks using traditional CNN search spaces does not give a good indication of their utility on more far-afield applications, which have often necessitated the design of custom neural operations \citep{cohen2018spherical,li2021fno}.

We make progress towards studying NAS on more diverse tasks by introducing a suite of benchmark datasets drawn from various data domains that we collectively call {\bf NAS-Bench-360}.
This benchmark consists of an organized setup of ten suitable datasets that (a) can be evaluated in a unified way using existing NAS approaches and (b) represent diverse application domains, dataset sizes, problem dimensionalities, and learning objectives.
We also include standard image classification evaluations as a baseline point of comparison, as many new methods continue to be designed for such tasks. 
NAS benchmarks typically involve precomputing all architectures in some fixed search space. In contrast, NAS-Bench-360 is explicitly intended to be agnostic of the search space being used---as different search spaces may work well for different tasks.\footnote{While NAS-Bench-360 is generally designed to be search space agnostic, we do provide precompute results using the NAS-Bench-201 search for specific analyses.} In this sense, NAS-Bench-360 is a task-oriented NAS benchmark with the intended use-case of evaluating NAS method and search space pairs on a wide variety of domains. 

% Rough overview of the types of analyses we'll show
%Experimentally, we demonstrate the usefulness of NAS-Bench-360 by performing a set of analyses evaluating whether the success of NAS in computer vision is indicative of strong performance on the much broader set of problems to which NAS can be applied. 
%First, we analyze the performance of various NAS methods\footnote{In this work, a {\em NAS method} is a combined search space and algorithm pair, not the algorithm alone.} and baselines under different budget constraints to simulate how practitioners in diverse domains might realistically apply deep learning methods to their tasks. Following this, we use the diverse tasks of NAS-Bench-360 to re-evaluate a series of NAS hypotheses from the literature that had been previously established for computer vision tasks. 

% Details and takeaways of the first analysis
%In our performance analyses of NAS methods and baselines on NAS-Bench-360, we ask whether modern NAS is even useful to practitioners when faced with a machine learning task from a diverse application domain. 
%To address this question, we start with the fact that a common first approach when applying deep learning to a new domain is to try an off-the-shelf CNN;
%in our case, this will be the Wide ResNet (WRN) \citep{zagoruyko2016wideresnet}. 
%We then consider two scenarios: (i) the practitioner is resource constrained and only has enough computational resources to train a single WRN using the default settings and (ii) the practitioner is less resource constrained, and has enough resources to tune WRN using an off-the-shelf hyperparameter optimizer \citep{li2018system}. Equalizing NAS methods with these baselines by their resource limits, we arrive at the following conclusions:
%\begin{itemize}[leftmargin=*,topsep=-1pt,noitemsep]\setlength\itemsep{2pt}
%	\item \textbf{In the more constrained setting (i)}, the practitioner is better off using WRN than NAS methods. 
%	\item \textbf{In the less constrained setting (ii)}, the practitioner might be better off using NAS methods, but risks catastrophic results on specific non-vision applications.
%\end{itemize}

% Details and takeaways of the second analysis
%In the sequel, we analyze NAS hypotheses from the literature and arrive at findings which contradict published claims in past NAS work, thus demonstrating the necessity and scientific value of NAS-Bench-360. 
%First, we include an analysis of a smaller, precomputed version of NAS-Bench-360 using the NAS-Bench-201 search space on two representatively diverse tasks selected from our benchmark. 
%Second, we evaluate of a zero-cost proxy method using the DARTS search space on these tasks and reinforce a recent analysis of zero-cost proxies on diverse tasks, including those in NAS-Bench-360 \cite{}.
%From these experiments, we arrive at the following surprising conclusions:
%\begin{itemize}[leftmargin=*,topsep=-1pt,noitemsep]\setlength\itemsep{2pt}
%	\item \textbf{Architecture rankings in NAS-Bench-201 vary drastically across diverse tasks.} The authors of NAS-Bench-201\citep{dong2020nasbench201} found that architecture ranking is consistent between their three vision tasks. We found that this phenomenon does not hold for diverse tasks. 
%	\item \textbf{The importance of different NAS operations varies drastically across diverse tasks.} Prior work \citep{wan2022on} has shown that the importance of different NAS operations for good performance is consistent across vision tasks. We found that this phenomenon also does not hold for diverse tasks. 
%	\item \textbf{NTK-based NAS is inconsistent across diverse classification tasks.} TE-NAS, a zero-cost proxy NAS method, claims to be able to identify high-performance architectures without training. We find that TE-NAS performs inconsistently on diverse classification tasks in NAS-Bench-360. 
%\end{itemize}



%Following our construction of this suite of tasks, we demonstrate both the usefulness of and need for NAS-Bench-360 by using it to investigate whether modern NAS is useful to practitioners faced with diverse tasks, i.e., whether its success in computer vision is indicative of strong performance on the much broader set of problems to which NAS can conceivably be applied.
%To address this question, we start with the fact that a common first approach when applying deep learning to a new domain is to try an off-the-shelf CNN;
%in our case, this will be the Wide ResNet (WRN) \citep{zagoruyko2016wideresnet}. 
%We then consider the scenario of two practitioners: 
%one with only the resources to train one WRN using the default settings and another that has enough resources to tune WRN using an off-the-shelf hyperparameter optimizer \citep{li2018system}.
%Both are faced with a decision:
%{\em should they use these fixed-architecture baselines or try out the best NAS has to offer?}

%Overall, our empirical investigation suggests the following:
%\begin{enumerate}[leftmargin=*,topsep=-1pt,noitemsep]\setlength\itemsep{2pt}
%	\item The less-constrained practitioner might usually do better using NAS---20\% relative improvement over WRN on the median task---but risks catastrophic results on specific non-vision applications.
%	\item The robustness of NAS in the constrained case may be worse:
%	the practitioner is likely better-off simply using the simple off-the-shelf WRN, as its median rank across NAS-Bench-360's ten tasks is the same as that of our candidate NAS method.
%\end{enumerate}
%These results are obtained via experiments using two well-studied modern search spaces: the cell-based DARTS space \citep{liu2019darts} and the efficiency-focused DenseNAS space \citep{fang2020densenas}.
%Each space is paired with a search method known to find well-performing architectures on ImageNet, specifically the state-of-the-art GAEA PC-DARTS \citep{li2021gaea} for the former and the original weight-sharing algorithm used by DenseNAS for the latter.
%Note that our assessment includes a more holistic comparison using performance profiles (c.f. Figure~\ref{fig:comparison}) to reinforce these ranking-based comparisons, which are useful but can miss a lack of robustness or exaggerate minor differences between methods.

%The initial experimental results enabled by NAS-Bench-360 suggest that the robustness of modern search methods to diverse tasks beyond image classification is mixed at best.
%At the same time, our set of tasks can serve as a crucial tool for investigating and rectifying this issue, and it is thus important for moving towards a truly automated pipeline containing NAS.
%In particular, NAS-Bench-360 will facilitate such progress via a diverse array of tasks for validating NAS methods that are not only challenging, real-life problem settings but also computationally accessible for academic researchers with limited budgets. 
%We demonstrate this potential via further studies on the comparative importance of search spaces vs. search algorithms, the usefulness of more-customized approaches, as well as strong transformer-based and non-deep learning baselines. 
%Specifically, we evaluate a random search (RS) baseline over the DenseNAS space, two domain-specific methods:
%Auto-DeepLab (Auto-DL) \citep{liu2019auto} for dense prediction and AMBER \citep{zhang2021automated} for prediction from 1D data, as well as the transformer-based Perceiver IO \citep{}, and XGBoost \citep{}.
%Among other insights, these experiments provide evidence that a more robust NAS may require better search spaces with a wider variety of operations.
 
 
%The initial experimental results enabled by NAS-Bench-360 suggest that the robustness of modern search methods to diverse tasks beyond image classification is mixed at best. At the same time, our set of tasks can serve as a crucial tool for investigating and rectifying this issue, and it is thus important for moving towards a truly automated pipeline containing NAS. In particular, NAS-Bench-360 will facilitate such progress via a diverse array of tasks for validating NAS methods that are not only challenging, real-life problem settings but also computationally accessible for academic researchers with limited budgets. 

We perform a thorough analysis of NAS methods and baselines on NAS-Bench-360, followed by a set of scientific analyses of published NAS findings originally demonstrated on computer vision tasks, and demonstrate that these analyses do not necessarily hold for diverse application domains. 

We have released all datasets, experiment code, seeds, and environments used in our experiments.\footnote{\url{https://github.com/rtu715/NAS-Bench-360}} 
Releasing our code, random seeds, and environments in the form of Docker containers assures reproducibility of all experimental results presented in this work and encourages the same level of reproducibility for future research performed using NAS-Bench-360. 


\begin{figure}[!t]
	
	\centering
	\includegraphics[width=0.47\linewidth]{figures/pp_fast.pdf}
	\includegraphics[width=0.47\linewidth]{figures/pp_slow.pdf}
	\caption{
		Performance profiles for two settings on all ten tasks in NAS-Bench-360.
		The y-value indicates the fraction of tasks on which a plotted method’s error is within a multiplicative factor $\tau$ of the lowest error achieved by all plotted methods, thus higher is better. 
	}
	\label{fig:comparison}
	
\end{figure}




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

